CryptoBap: A Binary Analysis Platform for Cryptographic Protocols

We introduce CryptoBap, a platform to verify weak secrecy and authentication for the (ARMv8 and RISC-V) machine code of cryptographic protocols. We achieve this by first transpiling the binary of protocols into an intermediate representation and then performing a crypto-aware symbolic execution to automatically extract a model of the protocol that represents all its execution paths. Our symbolic execution resolves indirect jumps and supports bounded loops using the loop-summarization technique, which we fully automate. The extracted model is then translated into models amenable to automated verification via ProVerif and CryptoVerif using a third-party toolchain. We prove the soundness of the proposed approach and used CryptoBap to verify multiple case studies ranging from toy examples to real-world protocols, TinySSH, an implementation of SSH, and WireGuard, a modern VPN protocol.

==> gfx/proof-overview.tex <==
\begin{figure*}
    \centering
\adjustbox{varwidth=\linewidth,scale=0.75}{%
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,178); %set diagram left start at 0, and has height of 178

%Rounded Rect [id:dp15033582439358972] 
\draw  [fill={rgb, 255:red, 161; green, 227; blue, 249 }  ,fill opacity=1 ] (0,143) .. controls (0,138.58) and (3.58,135) .. (8,135) -- (187,135) .. controls (191.42,135) and (195,138.58) .. (195,143) -- (195,167) .. controls (195,171.42) and (191.42,175) .. (187,175) -- (8,175) .. controls (3.58,175) and (0,171.42) .. (0,167) -- cycle ;
%Rounded Rect [id:dp49163767699067784] 
\draw  [fill={rgb, 255:red, 254; green, 213; blue, 172 }  ,fill opacity=1 ] (1,78.8) .. controls (1,73.39) and (5.39,69) .. (10.8,69) -- (94.2,69) .. controls (99.61,69) and (104,73.39) .. (104,78.8) -- (104,108.2) .. controls (104,113.61) and (99.61,118) .. (94.2,118) -- (10.8,118) .. controls (5.39,118) and (1,113.61) .. (1,108.2) -- cycle ;
%Rounded Rect [id:dp7748661947892861] 
\draw  [fill={rgb, 255:red, 161; green, 227; blue, 249 }  ,fill opacity=1 ] (1,10) .. controls (1,5.58) and (4.58,2) .. (9,2) -- (187,2) .. controls (191.42,2) and (195,5.58) .. (195,10) -- (195,34) .. controls (195,38.42) and (191.42,42) .. (187,42) -- (9,42) .. controls (4.58,42) and (1,38.42) .. (1,34) -- cycle ;
%Rounded Rect [id:dp8195126973531677] 
\draw  [fill={rgb, 255:red, 254; green, 213; blue, 172 }  ,fill opacity=1 ] (200,78) .. controls (200,73.58) and (203.58,70) .. (208,70) -- (233,70) .. controls (237.42,70) and (241,73.58) .. (241,78) -- (241,102) .. controls (241,106.42) and (237.42,110) .. (233,110) -- (208,110) .. controls (203.58,110) and (200,106.42) .. (200,102) -- cycle ;
%Straight Lines [id:da23355010731548242] 
\draw    (104,91) -- (197,91) ;
\draw [shift={(200,91)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp17131918646597977] 
\draw  [fill={rgb, 255:red, 254; green, 213; blue, 172 }  ,fill opacity=1 ] (320,78.6) .. controls (320,74.4) and (323.4,71) .. (327.6,71) -- (393.4,71) .. controls (397.6,71) and (401,74.4) .. (401,78.6) -- (401,101.4) .. controls (401,105.6) and (397.6,109) .. (393.4,109) -- (327.6,109) .. controls (323.4,109) and (320,105.6) .. (320,101.4) -- cycle ;
%Straight Lines [id:da47475691677265797] 
\draw    (241,90) -- (319,90) ;
\draw [shift={(322,90)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp6217318545676558] 
\draw  [fill={rgb, 255:red, 254; green, 213; blue, 172 }  ,fill opacity=1 ] (480,78.04) .. controls (480,74.15) and (483.15,71) .. (487.04,71) -- (508.16,71) .. controls (512.05,71) and (515.2,74.15) .. (515.2,78.04) -- (515.2,101.96) .. controls (515.2,105.85) and (512.05,109) .. (508.16,109) -- (487.04,109) .. controls (483.15,109) and (480,105.85) .. (480,101.96) -- cycle ;
%Straight Lines [id:da37929398674662385] 
\draw    (401,90) -- (460,90) -- (477,90) ;
\draw [shift={(480,90)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da5559609294522121] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (220,69) .. controls (322.96,-3.27) and (426.9,31.29) .. (491.07,69.83) ;
\draw [shift={(493,71)}, rotate = 211.36] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da7214008716902156] 
\draw    (196,26) -- (218.54,66.38) ;
\draw [shift={(220,69)}, rotate = 240.83] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da146309525901668] 
\draw    (195,151) -- (218.44,112.56) ;
\draw [shift={(220,110)}, rotate = 121.37] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Rounded Rect [id:dp779469587003883] 
\draw  [fill={rgb, 255:red, 254; green, 213; blue, 172 }  ,fill opacity=1 ] (579,78.6) .. controls (579,74.4) and (582.4,71) .. (586.6,71) -- (642.4,71) .. controls (646.6,71) and (650,74.4) .. (650,78.6) -- (650,101.4) .. controls (650,105.6) and (646.6,109) .. (642.4,109) -- (586.6,109) .. controls (582.4,109) and (579,105.6) .. (579,101.4) -- cycle ;
%Straight Lines [id:da6020724784951295] 
\draw    (516,91) -- (575,91) ;
\draw [shift={(578,91)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da6471890033093755] 
\draw    (229,132) -- (491,132) ;
\draw [shift={(491,132)}, rotate = 179.79] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)(-5.03,5.59) -- (-5.03,-5.59)   ;
\draw [shift={(229,132)}, rotate = 359.79] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)(-5.03,5.59) -- (-5.03,-5.59)   ;
%Straight Lines [id:da5145236549929502] 
\draw    (501,132) -- (619,132) ;
\draw [shift={(619,132)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)(-5.03,5.59) -- (-5.03,-5.59)   ;
\draw [shift={(501,132)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)(-5.03,5.59) -- (-5.03,-5.59)   ;

% Text Node
\draw (15,80) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{56.02pt}\setlength\topsep{0pt}
\small
\begin{center}
ARMv8 and\\RISC-V
\end{center}

\end{minipage}};
% Text Node
\draw (209,84) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\href{ssec:HolBA-framework}{BIR}};
% Text Node
\draw (6,5) node [anchor=north west][inner sep=0.75pt]   [align=left] {
Extended BIR semantics with \\
network communication Fig.\ref{birnetcom}
};
% Text Node
\draw (1,142) node [anchor=north west][inner sep=0.75pt]   [align=left] {
Cryptographic assumptions on\\
BIR program Definitions~\ref{rng-fun},~\ref{lib-fun} ,~\ref{ev-fun}
};
% Text Node
\draw (242,74) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Trace Inclusion}};
% Text Node
\draw (487,84.04) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {IML};
% Text Node
\draw (581,74) node [anchor=north west][inner sep=0.75pt]   [align=left] {
\small
CryptoVerif\\
\& ProVerif};
% Text Node
\draw (115,76) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Transpiler}};
% Text Node
\draw (112,94) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small \cite[Thm.~2]{DBLP:journals/scp/LindnerGM19}}};
% Text Node
\draw (323,74) node [anchor=north west][inner sep=0.75pt]   [align=left] {
\small
Crypto-aware\\
 Symb. Exec.
};
% Text Node
\draw (516,74) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Csec-modex}};
% Text Node
\draw (402,74) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Trace Inclusion}};
% Text Node
\draw (402,94) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small from Thm.~\ref{thm:iml:traceeq}}};
% Text Node
\draw (242,94) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small from Thm.~\ref{thm:bir:traceeq}}};
% Text Node
\draw (266,0) node [anchor=north west][inner sep=0.75pt]   [align=left] {
{\small Probability and Equality from Thm.\ref{thm:soundness} }\\
{\small using Thm.~\ref{thm:bir:traceeq}, Thm.~\ref{thm:iml:traceeq} and~\autoref{lem:thm4lems}}
};
% Text Node
\draw (500,110) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small \cite[Thm.~4.3,Thm.~5.2]{aizatulin_verifying_2020}}};
% Text Node
\draw (259,135) node [anchor=north west][inner sep=0.75pt]   [align=left] {
\small Using mixed IML-BIR semantics~\autoref{fig:mixedbiriml} and\\ IML-SBIR semantics~\autoref{fig:mixedsymbiml}
};
% Text Node
\draw (504,135) node [anchor=north west][inner sep=0.75pt]   [align=left] {\small Using IML semantics\\ \cite[p.~23]{aizatulin_verifying_2020}};
\end{tikzpicture}
}
    \caption{Proof overview}
    \label{fig:overview}
\end{figure*}


==> macros-bibcleanup.tex <==
\AtEveryBibitem{% Clean up the bibtex rather than editing it
 \clearlist{address}
 \clearfield{date}
 \clearlist{location}
 \clearfield{issn}
 \ifentrytype{book}{
  % \clearname{editor}
  }{}
\ifentrytype{inproceedings}{
  \clearname{editor}
  \clearfield{volume}
  \clearfield{url}
 \clearfield{isbn}
 \clearfield{month}
}{}
\ifentrytype{incollection}{
  \clearname{editor}
  \clearfield{volume}
  \clearfield{url}
 \clearfield{isbn}
 \clearfield{month}
}{}
\ifentrytype{proceedings}{
 \clearname{editor}
 \clearfield{volume}
 \clearfield{url}
 \clearfield{isbn}
 \clearfield{month}
}{}
\ifentrytype{article}{
 \clearfield{url}
 \clearfield{eprint}
 \clearfield{month}
 % \clearlist{publisher}
 % \clearfield{series}
 % \clearfield{volume}
}{}
}




==> macros-fulltricks.tex <==
\newcommand{\fullversionref}{trollthrottle-full}

\newcommand{\fref}[1]{\processifversion{conf}{F-}#1}
\newcommand{\fveqref}[1]{\processifversion{conf}{\eqref{F-#1}}\processifversion{full}{\eqref{#1}}}

\newcommand{\smallappendixorfull}[1]{%
\processifversion{conf}{\cite[App.~\ref{F-#1}]{\fullversionref}}%
\processifversion{full}{App.~\ref{#1}}%
}

\newcommand{\appendixorfull}[1]{%
\processifversion{conf}{extended
version~\cite[Appendix~\ref{F-#1}]{\fullversionref}}%
\processifversion{full}{Appendix~\ref{#1}}%
}
\newcommand{\theappendixorfull}[1]{%
\processifversion{conf}{the extended version~\cite[Appendix~\ref{F-#1}]{\fullversionref}}%
\processifversion{full}{Appendix~\ref{#1}}%
        }

% only cite in full version.
\newcommand{\fcite}[1]{%
\processifversion{conf}{}%
\processifversion{full}{~\cite{#1}}%
        }



==> sections/mixed_executions.tex <==
\section{Mixed executions}
\label{sec:imlmixexec}

So far, we can describe the correctness of the translation of a BIR
program into an IML process running in parallel to an attacker, but
not with other protocol parties.
%
In our SSH case study (cf. \autoref{sec:evaluation}), for instance,
the BIR program is an SSH server. 
Authentication, like many other protocol properties, encompasses
multiple parties. E.g., server authentication means that, whenever
\emph{the client} thinks they have established a connection with
a server, \emph{that same server} thinks they have connection with the
same client~\cite{woo1993semantic}. 
To achieve these properties, client and server share information,
e.g., the client knows the server key's fingerprint.

We thus lift our trace equivalence result to \ldots.


==> sections/mixed_executions_PSC.tex <==
\subsection{Mixed executions}
\label{sec:imlmixexec}

We describe the execution of a BIR program $\birprog$ in parallel to a
multiset of IML input processes $ \imlprocessq^{\mathit{full}} $ 
as a combination of the IML and BIR semantics via \emph{asynchronous
parallel composition}, a well-studied notion for system composition,
which we instantiate here, as follows.


\begin{definition}[asynchronous parallel composition]%
    \label{def:asynchronous-parallel-comp}
    The asynchronous parallel composition of two labelled transition systems with
    states $\stateSpace_i$, 
    initial state $\stateSpace^0_i\subseteq\stateSpace_i$,
    labels $\eventSpace$ and labelled transition
    relations $\rightarrow_i$ for $i=1,2$ is defined as a transition
    system with
    states $\stateSpace = \stateSpace_1 \times \stateSpace_2$,
    initial states $\stateSpace^0 = \stateSpace^0_1 \times \stateSpace^0_2$,
    labels $\eventSpace_1 \cup \eventSpace_2$ and
    $\rightarrow$ the smallest relation such that
    \begin{itemize}
        \item 
            $(c_1,c_2) \xrightarrow{e} (c_1',c_2')$
            if 
            $c_1\xrightarrow{e} c_1'$,
            $c_2\xrightarrow{e} c_2'$ 
            and 
            $a\in \eventSpace_1 \cap \eventSpace_2$,
        \item $(c_1,c_2) \xrightarrow{e}
             (c_1',c_2)$
             if $c_1 \xrightarrow{e}_2 c_1' \wedge e\notin \eventSpace_2$, and
        \item $(c_1,c_2) \xrightarrow{e}
            (c_1,c_2')$ if  $c_2 \xrightarrow{e} c_2' \wedge e\notin \eventSpace_1$.
    \end{itemize}
\end{definition}


% \begin{definition}[(symbolic) mixed execution]\label{def:mixed-execution} %{{{ 
%     The mixed (symbolic) BIR/IML execution 
%     is defined as a labelled transition system with state space
%     $\bitstates \times \imlstates$,
%     initial states \todo{Faezeh: please insert notation}
%     and
%     $\miximltrans{}{}{}{}{}$
%     the smallest relation such that
%     \begin{itemize}
%     \end{itemize}
%         \item 
%     $\miximltrans{}{}{}{\miximlstate{i}}{\miximlstateTwo{i+1}{j}}$
%     if
% $\birtrans{\Output{\overrightarrow{\var{e}}};\Input{\alpha}}{}{\birstate{i}}{\birstate{i+1}}$
% and
% there is a sequence of IML states such tat
% $
% \imltrans{}{}{\imlstate{i}}{\imlstate{i+1}}
% \cdots
% \imltrans{}{}{\imlstate{j-1}}{\imlstate{j}}
% $ 
% where the first and last transitions ...
% \item Allow IML and BIR transitions
% \end{definition}


We compose the IML and BIR semantics with the addition of a BIR
rule that synchronises with IML's \textsc{INew} rule.The purpose is
to allow the BIR program to share secrets with other processes in
$\imlprocessq^{\mathit{full}}$.

\begin{definition}[Mixed execution]\label{def:mixed-execution} %{{{ 
    The mixed execution of a BIR program $\birprog$ 
    and an IML program $\imlprog$ is the parallel composition of
    $\imltrans{}{}{}{}$
    and
    $\birtrans{}{x}{}{}$
    with 
    $\birtrans{}{x}{}{}$ defined as 
    $\birtrans{}{}{}{}$ with the additional rule:

    \begin{prooftree}
        \hypo{p\in[0,1]}
        \infer1[\textsc{Sync}]{ \birtrans{\imlfreshev{\var{x},\var{b}},p}
       {x}
       {\tuple{\birenv, \birpc}}
       {\tuple{\birenv [x \mapsto b], \birpc}}
   }
    \end{prooftree}

    To correctly incorporate IML's probabilities, we regard them as
    part of the transitions labels, hence \textsc{Sync}, the only
    synchronising step in BIR, carries the probability $p$. 
\end{definition}%}}}

\todo[inline]{Much easier if we can get probabilistic semantics for
    BIR.  Add the following rule as a middle step and split the
    uniform distribution lemma into two. Call this rBIR and add
    notation for it, e.g., \\rbirtrans.
    %
    I.e., BIR $\le$ vanilla-sBIR $\le$ sBIR $\le$ srBIR $\le$ IML.
}
\begin{prooftree}
    \hypo{ \begin{matrix}
       \birpc \in \lbls_{\mathcal{R}}\\
       \birpc'= \pcinc{\birpc}
	\end{matrix}}
	\hypo{\begin{matrix}
                p = 2^{-n}
                \\
		\eta' = \eta[\reg{0} \mapsto x; \randommemidx \mapsto \birenv.\randommemidx + \var{n}]       
    \end{matrix}}
	\infer2[RNG2($\var{n}$)]{\birprog\vdash \birtrans{\freshv{x}}{p}{\tuple{\birenv, \birpc}}{\tuple{{\birenv}', \birpc'}} }
\end{prooftree}

\begin{lemma}[Mixed BIR trace equivalence]
        For all  
        IML traces $\imlexecution \in \imlexecutions$,
        rBIR traces $\birexecution \in \birexecutions$
        and
        IML processes 
        $\imlprocessq^{\mathit{full}}$,
        if 
         $\simreltra{\sbirexecution}{\sbirvaluation}{\sbirtoiml{.}}{\imlexecution}$,

        % For all
        % mixed execution traces 
        % $\imlexecution' \in \mixedtraces(\imlprog, 
        % t

         $\simreltra{\sbirexecution}{P,\sbirvaluation}{\sbirtoiml{.}}{\imlexecution}$.
\end{lemma}
\begin{proof}
    Sketch:
    First show state equivalence. Modify eq relation to include
    equivalence of processes. Induction over transitions.
    All BIR rules: same as Lemma state eq.
    All IML rules: apply on both sides. (NOT TRUE, attacker knows
    more?)
    Extra BIR rule: TODO
\end{proof}


